Describe, Explain, Plan and Select: Interactive Planning with Large Language Models Enables Open-World Multi-Task Agents

We investigate the challenge of task planning for multi-task embodied agents in open-world environments. Two main difficulties are identified: 1) executing plans in an open-world environment (e.g., Minecraft) necessitates accurate and multi-step reasoning due to the long-term nature of tasks, and 2) as vanilla planners do not consider how easy the current agent can achieve a given sub-task when ordering parallel sub-goals within a complicated plan, the resulting plan could be inefficient or even infeasible. To this end, we propose "$\underline{D}$escribe, $\underline{E}$xplain, $\underline{P}$lan and $\underline{S}$elect" ($\textbf{DEPS}$), an interactive planning approach based on Large Language Models (LLMs). DEPS facilitates better error correction on initial LLM-generated $\textit{plan}$ by integrating $\textit{description}$ of the plan execution process and providing self-$\textit{explanation}$ of feedback when encountering failures during the extended planning phases. Furthermore, it includes a goal $\textit{selector}$, which is a trainable module that ranks parallel candidate sub-goals based on the estimated steps of completion, consequently refining the initial plan. Our experiments mark the milestone of the first zero-shot multi-task agent that can robustly accomplish 70+ Minecraft tasks and nearly double the overall performances. Further testing reveals our method's general effectiveness in popularly adopted non-open-ended domains as well (i.e., ALFWorld and tabletop manipulation). The ablation and exploratory studies detail how our design beats the counterparts and provide a promising update on the $\texttt{ObtainDiamond}$ grand challenge with our approach. The code is released at https://github.com/CraftJarvis/MC-Planner.

==> tables/ablation_feedback.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[h]
\caption{Success rates of DEPS under different maximum rounds of interactive feedback.}
\label{tab:ablation_on_feedback}
\renewcommand\arraystretch{1.1}
\begin{center}
\begin{tabular}{@{}cccccccc@{}}
\toprule
Rounds & 0 & 1 & 3 & 5 & $\infty$ & $\Delta(0\rightarrow \infty)$ \\ \midrule
MT1 & 28.6 & 50.6 & 68.1 & 79.8 & 79.8 & \textbf{+51.2} \\
MT2 & 37.1 & 71.2 & 71.4 & 79.2 & 79.5 & \textbf{+42.4} \\
MT3 & 15.1 & 20.1 & 40.3 & 40.8 & 62.4 & \textbf{+47.3} \\
MT4 & 15.9 & 17.4 & 48.3 & 50.7 & 53.3 & \textbf{+37.4} \\
MT5 & 3.2 & 3.2 & 3.2 & 15.2 & 29.2 & \textbf{+26.0} \\
MT6 & 0.5 & 0.5 & 1.1 & 1.9 & 13.8 & \textbf{+13.3} \\
MT7 & 0.6 & 2.3 & 2.9 & 2.9 & 12.6 & \textbf{+12.0} \\
MT8 & 0.0 & 0.0 & 0.0 & 0.0 & 0.6 & \textbf{+0.6} \\ \bottomrule
\end{tabular}
\vskip -0.2in
\end{center}
\end{table}

==> tables/ablation_goal_model.tex <==
% \begin{table*}
% \caption{Success rate of different goal-model under different number of goals and different maximum episode length.}
% \label{tab:ablation_goals}
% \centering
%  \begin{minipage}[t]{0.3\textwidth}
%   \centering
%      %\makeatletter\def\@captype{table}\makeatother\caption{Goal-Model under 600 Eps.}
%      \resizebox{\linewidth}{!}{
%         \renewcommand\arraystretch{1.1}
%        \begin{tabular}{@{}lcccc@{}}
%             \toprule
%             Goal-Model & 1    & 2    & 3    & 4   \\ \midrule
%             Fixed      & 43.0 & 12.0 & 4.0  & 2.0 \\
%             Random     & 43.0 & 15.0 & 5.0  & 1.0 \\
%             MINECLIP   & 47.0 & 10.0 & 3.0  & 0.0 \\
%             % CLIP       & 0.0  & 0.0  & 0.0  & 0.0 \\
%             HPGM       & \textbf{49.0} & \textbf{21.0} & \textbf{14.0} & \textbf{2.0} \\ \bottomrule
% \end{tabular}
% }
%   \end{minipage}
%   \begin{minipage}[t]{0.3\textwidth}
%    \centering
%     %\makeatletter\def\@captype{table}\makeatother\caption{Goal-Model under 1200 Eps.}
%     \resizebox{\linewidth}{!}{
% \renewcommand\arraystretch{1.1}
%        \begin{tabular}{@{}lcccc@{}}
%             \toprule
%             Goal-Model & 1    & 2    & 3    & 4    \\ \midrule
%             Fixed      & \textbf{62.0} & 28.0 & 10.0 & 6.0  \\
%             Random     & 54.0 & 24.0 & 16.0 & 4.0  \\
%             MINECLIP   & 61.0 & 17.0 & 12.0 & 1.0  \\
%             % CLIP       & 0.0  & 0.0  & 0.0  & 0.0  \\
%             HPGM       & 58.0 & \textbf{33.0} & \textbf{30.0} & \textbf{12.0} \\ \bottomrule
% \end{tabular}
% }
%    \end{minipage}
%    \begin{minipage}[t]{0.3\textwidth}
%    \centering
%     %\makeatletter\def\@captype{table}\makeatother\caption{Goal-Model under 2400 Eps.}
%     \resizebox{\linewidth}{!}{
% \renewcommand\arraystretch{1.1}
%        \begin{tabular}{@{}lcccc@{}}
%             \toprule
%             Goal-Model & 1    & 2    & 3    & 4    \\ \midrule
%             Fixed      & 69.0 & 38.0 & 15.0 & 11.0 \\
%             Random     & 68.0 & 32.0 & 26.0 & 15.0 \\
%             MINECLIP   & \textbf{75.0} & 25.0 & 18.0 & 4.0  \\
%             % CLIP       & 0.0  & 0.0  & 0.0  & 0.0  \\
%             HPGM       & 72.0 & \textbf{42.0} & \textbf{45.0} & \textbf{22.0} \\ \bottomrule
% \end{tabular}
% }
%    \end{minipage}
% \end{table*}

% \begin{figure}[t]
%     \centering
%     \includegraphics[scale = 0.4]{figures/ablation_goalmodel_2.pdf}
%     \caption{
%         \textbf{Ablation experiments on different Selector implementations}.
%         The success rates of different selectors under varying numbers of parallel goals and maximum episode lengths.}
%     \label{fig:ablation_goalmodel}
%     \vskip -0.2in
% \end{figure}



==> tables/milestone.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[H]
\centering
\caption{Success rate of milestone items for mining diamond.}
\label{tab:milestone_succ}
\renewcommand\arraystretch{1.1}
\begin{tabular}{cc}
\toprule
milestone items & success rate \\ \midrule
log & 96.70$\pm$2.04 \\
planks & 88.98$\pm$0.95 \\
stick & 88.98$\pm$0.95 \\
crafting\_table & 88.98$\pm$0.95 \\
wooden\_pickaxe & 86.47$\pm$1.38 \\
cobblestone & 83.14$\pm$1.87 \\
furnace & 68.66$\pm$2.46 \\
stone\_pickaxe & 67.90$\pm$2.77 \\
iron\_ore & 31.59$\pm$7.81 \\
iron\_ingot & 8.85$\pm$2.58 \\
iron\_pickaxe & 8.69$\pm$2.79 \\
diamond & 0.59$\pm$0.52 \\ \bottomrule
\end{tabular}
\end{table}

==> tables/task_list.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[t]
\caption{Full task list of every meta task in Minecraft TASK101.}
\label{tab:task_list}
\resizebox{\linewidth}{!}{
\renewcommand\arraystretch{1.2}
\begin{tabular}{@{}ccccccc@{}}
\toprule
Meta-Task & Task & \begin{tabular}[c]{@{}c@{}}Reasoning\\ Steps\end{tabular} & Object & Task & \begin{tabular}[c]{@{}c@{}}Reasoning\\ Steps\end{tabular} & Object \\ \midrule
\multirow{7}{*}{\begin{tabular}[c]{@{}c@{}}MT1\\ Basic\end{tabular}} & \texttt{CraftPlanks} & 2 & planks & \texttt{CraftOakStairs} & 4 & oak\_stairs \\
 & \texttt{CraftSticks} & 3 & stick & \texttt{CraftSign} & 5 & sign \\
 & \texttt{CraftWoodenSlab} & 4 & wooden\_slab & \texttt{CraftFence} & 5 & fence \\
 & \texttt{CraftWoodenPressurePlate} & 3 & wooden\_pressure\_plate & \texttt{CraftFenceGate} & 5 & fence\_gate \\
 & \texttt{CraftBowl} & 4 & bowl & \texttt{CraftBoat} & 4 & boat \\
 & \texttt{CraftWoodenButton} & 3 & wooden\_button & \texttt{CraftTrapdoor} & 4 & trapdoor \\
 & \texttt{CraftChest} & 4 & chest & \texttt{CraftWoodenDoor} & 4 & wooden\_door \\ \midrule
 \multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}MT2\\ Tool\\ (Simple)\end{tabular}} & \texttt{CraftCraftingTable} & 3 & crafting\_table & \texttt{CraftFurnace} & 7 & furnace \\
 & \texttt{CraftWoodenPickaxe} & 5 & wooden\_pickaxe & \texttt{CraftStonePickaxe} & 7 & stone\_pickaxe \\
 & \texttt{CraftWoodenAxe} & 5 & wooden\_axe & \texttt{CraftStoneAxe} & 7 & stone\_axe \\
 & \texttt{CraftWoodenHoe} & 5 & wooden\_hoe & \texttt{CraftStoneHoe} & 7 & stone\_hoe \\
 & \texttt{CraftWoodenSword} & 5 & wooden\_sword & \texttt{CraftStoneShovel} & 7 & stone\_shovel \\
 & \texttt{CraftWoodenShovel} & 5 & wooden\_shovel & \texttt{CraftStoneSword} & 7 & stone\_sword \\ \midrule
 \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}MT3\\ Hunt \\ \& Food\end{tabular}} & \texttt{CraftBed} & 5 & bed & \texttt{CookPorkchop} & 9 & cooked\_porkchop \\
 & \texttt{CraftPainting} & 6 & painting & \texttt{CookBeef} & 9 & cooked\_beef \\
 & \texttt{CraftCarpet} & 5 & carpet & \texttt{CookMutton} & 9 & cooked\_mutton \\
 & \texttt{CraftItemFrame} & 6 & item\_frame &  &  &  \\ \midrule
\multirow{7}{*}{\begin{tabular}[c]{@{}c@{}}MT4\\ Dig-Down\end{tabular}} & \texttt{CraftStoneStairs} & 7 & stone\_stairs & \texttt{CraftStoneBrick} & 9 & stone\_brick  \\
 & \texttt{CraftStoneSlab} & 7 & stone\_slab & \texttt{CraftTorch} & 9 & torch \\
 & \texttt{CraftArmorStand} & 10 & armor\_stand & \texttt{ObtainCoal} & 8 & coal \\
 & \texttt{CraftCobblestoneWall} & 7 & cobblestone\_wall & \texttt{CraftStoneBrickStairs} & 10 & stonebrick\_stairs \\
 & \texttt{CraftQuartzBlock} & 10 & quartz\_block & \texttt{CraftStonePressurePlate} & 9 & stone\_pressure\_plate \\
 & \texttt{CraftStoneBrick} & 9 & stonebrick & \texttt{CraftStoneButton} & 7 & stone\_button \\
 & \texttt{SmeltStone} & 9 & stone & \texttt{CraftLever} & 7 & level \\ \midrule
\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}MT5\\Equipment\end{tabular}} & \texttt{EquipLeatherBoots} & 5 & leather\_boots & \texttt{EquipIronChestplate} & 11 & iron\_chestplate \\
 & \texttt{EquipLeatherChestplate} & 5 & leather\_chestplate & \texttt{EquipIronLeggings} & 11 & iron\_leggings \\
 & \texttt{EquipLeatherHelmet} & 5 & leather\_helmet & \texttt{EquipIronHelmet} & 11 & iron\_helmet \\
 & \texttt{EquipLeatherLeggings} &  5 & leather\_leggings & \texttt{EquipIronBoots} & 11 & iron\_boots \\
 & \texttt{EquipShield} & 11 & shield &  &  &  \\ \midrule
 \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}MT6\\ Tool\\ (Complex)\end{tabular}} & \texttt{CraftBucket} & 11 & bucket & \texttt{CraftIronHoe} & 11 & iron\_hoe \\
 & \texttt{CraftShears} & 11 & shears & \texttt{CraftIronShovel} & 11 & iron\_shovel \\
 & \texttt{CraftIronPickaxe} & 11 & iron\_pickaxe & \texttt{CraftIronSword} & 11 & iron\_sword \\
 & \texttt{CraftIronAxe} & 11 & iron\_axe &  &  &  \\ \midrule
\multirow{7}{*}{\begin{tabular}[c]{@{}c@{}}MT7\\Iron-Stage \end{tabular}} & \texttt{CraftIronBars} & 11 & iron\_bars & \texttt{CraftChestMinecart} & 13 & chest\_minecart \\
 & \texttt{CraftIronNugget} & 11 & iron\_nugget & \texttt{CraftIronDoor} & 11 &  iron\_door \\
 & \texttt{CraftMinecart} & 11 & minecart & \texttt{CraftIronTrapdoor} & 11 & iron
 \_trapdoor \\
 & \texttt{CraftHopper} & 12 & hopper & \texttt{CraftTripwireHook} & 11 & tripwire\_hook \\
 & \texttt{CraftHopperMinecart} & 14 & hopper\_minecart & \texttt{CraftHeavyWeightedPressurePlate} & 11 & heavy\_weighted\_pressure\_plate \\
 & \texttt{CraftFurnaceMinecart} & 12 & furnace\_minecart & \texttt{CraftRail} & 11 & rail \\
 & \texttt{CraftCauldron} & 11 & cauldron &  &  &  \\ \midrule
\multicolumn{1}{l}{\begin{tabular}[c]{@{}c@{}}Challenge\\ MT8\end{tabular}} & \texttt{MineDiamond} & 12 & diamond &  &  &  \\  \bottomrule 
\end{tabular}}
\end{table}
